IteraOptiRacing: A Unified Planning-Control Framework for Real-time Autonomous Racing for Iterative Optimal Performance

This paper presents a unified planning-control strategy for competing with other racing cars called IteraOptiRacing in autonomous racing environments. This unified strategy is proposed based on Iterative Linear Quadratic Regulator for Iterative Tasks (i2LQR), which can improve lap time performance in the presence of surrounding racing obstacles. By iteratively using the ego car's historical data, both obstacle avoidance for multiple moving cars and time cost optimization are considered in this unified strategy, resulting in collision-free and time-optimal generated trajectories. The algorithm's constant low computation burden and suitability for parallel computing enable real-time operation in competitive racing scenarios. To validate its performance, simulations in a high-fidelity simulator are conducted with multiple randomly generated dynamic agents on the track. Results show that the proposed strategy outperforms existing methods across all randomly generated autonomous racing scenarios, enabling enhanced maneuvering for the ego racing car.

==> sections/bio.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-photo/ieee_photo_yifan.jpg}}]{Yifan Zeng} received his B.Eng. degree in Mechanical Engineering from Shanghai Jiao Tong University, Shanghai, China, in 2021. He obtained the M.Eng. degree in Mechanical Engineering from Shanghai Jiao Tong University, Shanghai, China, in 2024.
 
    His research interests lie in the fields of robotics and autonomous vehicles, with a particular focus on planning and control.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-photo/ieee_photo_yihan.png}}]{Yihan Li} received her B.Eng. degree in Automation from Xi'an Jiaotong University, Xi'an, China, in 2024. She is currently a master student in Robotics in GRASP Lab at University of Pennsylvania, Philadelphia, USA. Her research interests lie in trajectory generation and optimization, planning and imitation learning.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-photo/ieee_photo_suiyi.png}}]{Suiyi He} received B.Eng. degrees in Mechatronics from both Tongji University, Shanghai, China and Hochschule Esslingen, Esslingen a.N., Germany, in 2019. He obtained the M.Eng. degree in Robotics from the University of California, Berkeley, USA, in 2020. Currently, he is a Ph.D. candidate in the Department of Mechanical Engineering at the University of Minnesota, Minneapolis, USA. His research interests lie at the intersection of optimization, planning and control with applications in connected and autonomous vehicles.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-photo/ieee_photo_koushil.png}}]{Koushil Sreenath} received the M.S. degree in Applied Mathematics and the Ph.D. degree in Electrical Engineering and Systems from the University of Michigan, Ann Arbor, MI, USA, in 2011. He is an Assistant Professor of Mechanical Engineering with the University of California, Berkeley, Berkeley, CA, USA. He was an Assistant Professor with Carnegie Mellon University, Pittsburgh, PA, USA, between 2013 and 2017. His research interests include the intersection of highly dynamic robotics and applied nonlinear control.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-photo/ieee_photo_jun.png}}]{Jun Zeng} received his Ph.D. in Control and Robotics from the Department of Mechanical Engineering at the University of California, Berkeley, USA, in 2022, his Dipl. Ing. degree from École Polytechnique, France, in 2017, and his B.S.E. degree from Shanghai Jiao Tong University, China, in 2016. His research interests lie at the intersection of optimization, control, planning, and learning, with applications to various robotics platforms.
\end{IEEEbiography}

